Augmented Neural Ordinary Differential Equations for Power System Identification

Due the complexity of modern power systems, modeling based on first-order principles becomes increasingly difficult. As an alternative, dynamical models for simulation and control design can be obtained by black-box identification techniques. One such technique for the identification of continuous-time systems are neural ordinary differential equations. For training and inference, they require initial values of system states, such as phase angles and frequencies. While frequencies can typically be measured, phase angle measurements are usually not available. To tackle this problem, we propose a novel structure based on augmented neural ordinary differential equations, learning latent phase angle representations on historic observations with temporal convolutional networks. Our approach combines state-of-the art deep learning techniques, avoiding the necessity of phase angle information for the power system identification. Results show, that our approach clearly outperforms simpler augmentation techniques.

==> figures/newNodeCommands.tex <==
% !TeX encoding = UTF-8
% !TeX spellcheck = en_GB
% !TEX TS-program = pdflatex
% !TEX root = ../book.tex

\newcommand{\lnwidth}{0.65pt}
% \newcommand{\lngrid}{0.5pt}
\newcommand{\scaleSymbols}{0.035}

\newcommand{\GraphLine}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
	\path[line join=miter,line cap=round,miter limit=4.00,rounded corners=0.0000cm] (0,0)
	rectangle (24,1);
	\path[draw] (7, 0.5) -- (17, 0.5);
	\end{tikzpicture}}

\newcommand{\GraphLineFlip}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex, rotate=90]
	\path[line join=miter,line cap=round,miter limit=4.00, rounded corners=0.0000cm] (0,0)
	rectangle (24,1);
	\path[draw] (7, 0.5) -- (17, 0.5);
	\end{tikzpicture}}

\newcommand{\GraphTransformer}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
	\path[line join=miter,line cap=round,miter limit=4.00, rounded corners=0.0000cm] (0,0)
	rectangle (24,24);
	\path[draw=none, fill=white] (12, 15) circle (6);
	\path[draw, fill=white] (12, 9) circle (6);
	\path[draw] (12, 15) circle (6);
	\end{tikzpicture}}

\newcommand{\GraphTransformerFlip}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex, rotate=90]
	\path[line join=miter,line cap=round,miter limit=4.00, rounded corners=0.0000cm] (0,0)
	rectangle (24,24);
	\path[draw=none, fill=white] (12, 15) circle (6);
	\path[draw, fill=white] (12, 9) circle (6);
	\path[draw] (12, 15) circle (6);
	\end{tikzpicture}}

\newcommand{\GraphInverter}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
	\path[line join=miter, line cap=round, miter limit=4.00, line width=\lnwidth,
			rounded corners=0.0000cm] (0,0) rectangle (24,24);
	\path[draw, line join=miter, line cap=butt, miter limit=4.00, line width=\lnwidth] (22, 2) -- (2, 22);
	\draw [line width=\lnwidth] plot [smooth, tension=1] coordinates { (21, 19) (18, 16) (15, 19) (12, 16)};
	\draw [line width=\lnwidth]
		(4, 5.25) -- (11, 5.25)
		(4, 7.75) -- (11, 7.75);
	\end{tikzpicture}}

\newcommand{\GraphInverterFlip}{\begin{tikzpicture}[scale = \scaleSymbols*20/24, >=latex]
	\path[line join=miter, line cap=round, miter limit=4.00, line width=\lnwidth,
	rounded corners=0.0000cm] (0,0) rectangle (24,24);
	\path[draw, line join=miter, line cap=butt, miter limit=4.00, line width=\lnwidth] (22, 2) -- (2, 22);
	\draw [line width=\lnwidth] plot [smooth, tension=1] coordinates { (21, 19) (18, 16) (15, 19) (12, 16)};
	\draw [line width=\lnwidth]
	(4, 5.25) -- (11, 5.25)
	(4, 7.75) -- (11, 7.75);
	\end{tikzpicture}}

\newcommand{\tower}{\begin{tikzpicture}[scale = \scaleSymbols*20/24, >=latex]
      \path[line join=miter,line cap=round,miter
         limit=4.00,line width=\lnwidth,rounded corners=0.0000cm]
				(0,0)
       rectangle (24,24);
   \draw (-1,0) arc (180:360:1cm and 0.5cm);
    \draw (-1,0) arc (180:0:1cm and 0.5cm);
    \draw (-2,-3) arc (180:360:2cm and 1cm);
    %\draw[dashed] (-2,-3) arc (180:10:2cm and 1cm);
    \draw(-2,-3)  -- (-1,0);
    \draw(2,-3)   -- (1,0);
    \shade[left color=blue!5!white,right color=blue!60!white,opacity=0.3] (-1,0) arc (180:360:1cm and 0.5cm) -- (2,-3) arc (360:180:2cm and 1cm) -- cycle;
    \shade[left color=blue!5!white,right color=blue!60!white,opacity=0.3] (0,0) circle (1cm and 0.5cm);
\end{tikzpicture}
}

\newcommand{\GraphTristateTF}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
      \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (0,0)
        rectangle (24,24);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (0,12) -- (4,12);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (20,12) -- (24,12);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (15,12) circle (5);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (9,12) circle (5);
\end{tikzpicture}}

\newcommand{\GraphTristatePCC}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
      \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (0,0)
        rectangle (24,24);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (0,12) -- (9,12) -- (15,6);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (15,12) -- (24,12);
\end{tikzpicture}}

\newcommand{\GraphTristateR}{
%	\renewcommand{\linewidthR}m}
\begin{tikzpicture}[scale = \scaleSymbols, >=latex, color=black]
        \path[] (315.0000,52.3622-1) rectangle (335.0000,72.3622-1);
        \path[draw,fill,line join=round,line cap=round,miter limit=4.00,line
          width=1.5*\lnwidth] (324.0306,59.8874) .. controls (321.9302,58.2551) and
          (319.7014,56.9114) .. (317.2333,55.6929) .. controls (319.8093,57.9660) and
          (324.1469,60.6035) .. (324.0306,59.8874) -- cycle;
        \path[draw,fill,line join=round,line cap=round,miter limit=4.00,line
          width=1.5*\lnwidth] (325.5865,60.4167) .. controls (328.0392,59.6017) and
          (330.4240,58.6404) .. (332.7667,57.0558) .. controls (329.8032,57.9971) and
          (326.8503,59.6115) .. (325.5865,60.4167) -- cycle;
        \path[draw,fill,line join=round,line cap=round,miter limit=4.00,line
          width=1.5*\lnwidth] (324.8607,61.1176) .. controls (324.6795,63.5961) and
          (324.6662,66.1651) .. (325.3315,69.0315) .. controls (325.5549,66.1044) and
          (325.1090,62.6873) .. (324.8607,61.1176) -- cycle;
        \path[cm={{0.20207,0.0904,-0.09626,0.21517,(296.36236,26.26027)}},draw,fill,line
          join=round,line cap=round,miter limit=4.00,line width=2*\lnwidth]
          (186.0000,84.3622) .. controls (186.0000,86.6957) and (183.5376,88.5874) ..
          (180.5000,88.5874) .. controls (177.4624,88.5874) and (175.0000,86.6957) ..
          (175.0000,84.3622) .. controls (175.0000,82.0287) and (177.4624,80.1370) ..
          (180.5000,80.1370) .. controls (183.5376,80.1370) and (186.0000,82.0287) ..
          (186.0000,84.3622) -- cycle;
\end{tikzpicture}
}

%===================

\newcommand{\GraphTristateS}{
\begin{tikzpicture}[scale = -\scaleSymbols, >=latex, color=black]
        \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (265.0000,52.3622)
          rectangle (285.0000,72.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (269.0000,61.3622) -- (281.0000,61.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (275.0000,55.3622) -- (275.0000,61.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (272.0000,63.3622) -- (278.0000,63.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (275.0000,63.3622) -- (275.0000,69.3622);
\end{tikzpicture}
}


% %===================

\newcommand{\GraphTristateT}{
\begin{tikzpicture}[scale = -\scaleSymbols, >=latex, color=black]
        \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (495.0000,52.3622-.5)
          rectangle (515.0000,72.3622-.5);
        \path[cm={{0.38462,0.0,0.0,0.83333,(380.9615,-59.27301)}},draw, line
          join=round,line cap=round,miter limit=4.00,line width=\lnwidth, color = black]
          (342.0000,145.3622) .. controls (342.0000,150.3328) and (333.2695,154.3622) ..
          (322.5000,154.3622) .. controls (311.7305,154.3622) and (303.0000,150.3328) ..
          (303.0000,145.3622) .. controls (303.0000,140.3916) and (311.7305,136.3622) ..
          (322.5000,136.3622) .. controls (333.2695,136.3622) and (342.0000,140.3916) ..
          (342.0000,145.3622) -- cycle;
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth, color = black]
          (505.0000,54.3622) -- (505.0000,69.3622);
\end{tikzpicture}
}


% %===================

\newcommand{\GraphTristateP}{
\begin{tikzpicture}[scale = -\scaleSymbols, >=latex, color=black]
        \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (495.0000,52.3622)
          rectangle node {N} (515.0000,72.3622) ;
\end{tikzpicture}
}

% %===================

\newcommand{\GraphTristatePV}{
\begin{tikzpicture}[scale =  -\scaleSymbols, >=latex, color=black]
%=== PV ===
  \begin{scope}[cm={{1.33333,0.0,0.0,1.33333,(-219.66665,-77.45405)}}]
    \path[line join=miter,line cap=round,miter
      limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (371.0000,157.3622)
      rectangle (386.0000,172.3622);
    \begin{scope}[cm={{0.75,0.0,0.0,0.75,(108.84792,54.02778)}}]
      \path[cm={{0.45455,0.21485,-0.21652,0.51139,(295.25671,66.03768)}},draw=white,fill,line
        join=round,line cap=round,miter limit=4.00,line width=1*\lnwidth]
        (186.0000,84.3622) .. controls (186.0000,86.6957) and (183.5376,88.5874) ..
        (180.5000,88.5874) .. controls (177.4624,88.5874) and (175.0000,86.6957) ..
        (175.0000,84.3622) .. controls (175.0000,82.0287) and (177.4624,80.1370) ..
        (180.5000,80.1370) .. controls (183.5376,80.1370) and (186.0000,82.0287) ..
        (186.0000,84.3622) -- cycle;
      \begin{scope}[shift={(-0.46388,0.41703)}]
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (362.2097,144.9631) -- (368.0000,139.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,151.3622) -- (356.4103,149.0251);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (363.3146,147.2675) -- (368.0000,147.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,143.3622) -- (356.1804,145.6575);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (368.0000,155.3622) -- (362.5254,149.6350);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (358.2954,144.1423) -- (356.0000,139.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (360.0000,155.3622) -- (359.9369,151.0555);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,155.3622) -- (357.0000,150.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,147.3622) -- (356.2119,147.4569);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,139.3622) -- (357.1274,144.7105);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (359.8422,144.3002) -- (360.0000,139.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (361.3258,144.2370) -- (364.0000,139.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (356.0000,155.3622) -- (358.2954,150.8977);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (362.6832,145.9732) -- (368.0000,142.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (363.2514,148.3092) -- (368.0000,149.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (364.6693,154.2802) -- (361.4307,150.5189);
      \end{scope}
    \end{scope}
  \end{scope}
\end{tikzpicture}
}

